CSP: A Simulator For Multi-Agent Ranking Competitions

In ranking competitions, document authors compete for the highest rankings by modifying their content in response to past rankings. Previous studies focused on human participants, primarily students, in controlled settings. The rise of generative AI, particularly Large Language Models (LLMs), introduces a new paradigm: using LLMs as document authors. This approach addresses scalability constraints in human-based competitions and reflects the growing role of LLM-generated content on the web-a prime example of ranking competition. We introduce a highly configurable ranking competition simulator that leverages LLMs as document authors. It includes analytical tools to examine the resulting datasets. We demonstrate its capabilities by generating multiple datasets and conducting an extensive analysis. Our code and datasets are publicly available for research.

==> ack.tex <==
% \smallskip
% \myparagraph{Acknowledgments} We thank the reviewers for their comments.
% The work by Moshe Tennenholtz was supported by funding from the
% European Research Council (ERC) under the European Union's Horizon
% 2020 research and innovation programme (grant agreement 740435).


==> category.tex <==
% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10002951</concept_id>
% <concept_desc>Information systems</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002951.10003317</concept_id>
% <concept_desc>Information systems~Information retrieval</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002951.10003317.10003338</concept_id>
% <concept_desc>Information systems~Retrieval models and ranking</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Information systems}
% \ccsdesc[500]{Information systems~Information retrieval}
% \ccsdesc[500]{Information systems~Retrieval models and ranking}


% \keywords{competitive search, ranking-incentivized manipulations, adversarial retrieval}


\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002951</concept_id>
       <concept_desc>Information systems</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003317</concept_id>
       <concept_desc>Information systems~Information retrieval</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003317.10003365</concept_id>
       <concept_desc>Information systems~Search engine architectures and scalability</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003317.10003365.10010850</concept_id>
       <concept_desc>Information systems~Adversarial retrieval</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems}
\ccsdesc[500]{Information systems~Information retrieval}
\ccsdesc[500]{Information systems~Search engine architectures and scalability}
\ccsdesc[500]{Information systems~Adversarial retrieval}

\keywords{competitive search, LLM, simulation, agents}


==> prompts_and_confs/str_conf.tex <==
\begin{minted}[breaklines=true, fontsize=\scriptsize, frame=lines, tabsize=2]{json}
{
    "competition": {
        "round_by_round": true,
        "init_docs_path": {
            "queries_folder_path": "data/web_track",
            "docs_file_path": "data/initial_documents.trectext"
        },
        "rankers": {
            "e5": {
                "model_name": "intfloat/e5-large-unsupervised"
            }
        },
        "llm": {
            "model_name": "google/gemma-2-9b-it",
            "token": "<HF_TOKEN>",
            "temperature": 0.5,
            "top_p": 0.9
        }
    },
    "game": {
        "max_tokens": 256,
        "rounds": 30,
        "force_max_tokens": true
    },
    "agents": {
    "student": {
        "character": "behave like a BSc student",
        "prompt_format": "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles.\n",
        "pairwise": false,
        "depth": 2
    },
    "writer": {
        "character": "behave like a professional writer",
        "prompt_format": "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles.\n",
        "pairwise": false,
        "depth": 2
    },
    "editor": {
        "character": "behave like a professional editor",
        "prompt_format": "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles.\n",
        "pairwise": false,
        "depth": 2
    },
    "teacher": {
        "character": "behave like an English teacher",
        "prompt_format": "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles.\n",
        "pairwise": false,
        "depth": 2
    },
    "professor": {
        "character": "behave like a Data Science professor",
        "prompt_format": "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles.\n",
        "pairwise": false,
        "depth": 2
    }
}
}
\end{minted}

==> prompts_and_confs/str_prompt_clean.tex <==
\begin{minted}[breaklines=true, frame=single, fontsize=\small]{python}
CLEANING_PROMPT = "Your task is to clean up the document generated by an LLM. Remove any headers, prefixes, or metadata such as \"This is the modified document\" or similar phrases that are not part of the actual content. Exclude statements that describe how the document was modified or its characteristics, such as its length or ranking. Specifically, omit sentences like the following:\n\n- [The text above is the extracted document part.]\n- The extracted document part:\n- [The document text remains unchanged.]\n- (The extracted document part ends here)\n- [Document text only, no modifications or additions made.]\n- [End of Document]\n- [The rest of the text is not the document part and will be ignored.]\n- [Document Text Only]\n- *Here is the document text you requested, unaltered:*\n- To improve the ranking\n- the document length is 147 words\n\nImportant: Do not change or modify the actual content of the document. Only remove unnecessary prefixes, headers, or metadata, leaving the original text of the document untouched and unaltered. The output should read naturally, without unnecessary formatting or markers."
\end{minted}

==> prompts_and_confs/str_prompt_listwise.tex <==
\begin{minted}[breaklines=true, frame=single, fontsize=\small]{python}
LISTWISE_PROMPT = "\n\nquery: <QUERY>\n\n* documents ordered by latest ranking from highest to lowest in relation to the query: \n\n\n* <DOCUMENT a>\n\n\n* <DOCUMNET b>\n\n\n* <DOCUMENT c>\n\n\n* <DOCUMENT d>\n\n\n\n\n\n * documents ranked by second to latest ranking from highest to lowest in relation to the query:\n1. <DOCUMENT e>\n2. <DOCUMENT f>\n3. <DOCUMENT g>\n4. <DOCUMENT h>\n5. <DOCUMENT i>\n\n\n\n"
\end{minted}

==> prompts_and_confs/str_prompt_pairwise.tex <==
\begin{minted}[breaklines=true, frame=single, fontsize=\small]{python}
PAIRWISE_PROMPT = "\n\nquery: <QUERY>\n\n* document: <DOCUMENT a>\n\nlatest ranking: <RANK r(a)>\n\n\n* document: <DOCUMENT b>\n\nlatest ranking: <RANK r(b)>\n\n\n\n\nquery: <QUERY>\n\n* document: <DOCUMENT c>\n\nsecond to latest ranking: <RANK r(c)>\n\n\n* document: <DOCUMENT d>\n\nsecond to latest ranking: <RANK r(d)>\n\n\n\n\nquery: <QUERY>\n\n* document: <DOCUMENT e>\n\nthird to latest ranking: <RANK r(e)>\n\n\n* document: <DOCUMENT f>\n\nthird to latest ranking: <RANK r(f)>"
\end{minted}

==> prompts_and_confs/str_prompt_system.tex <==
\begin{minted}[breaklines=true, frame=single, fontsize=\small]{python}
SYSTEM_PROMPT = "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles. \n Input: \n\n - Candidate Query: <QUERY> \n\n - Candidate Document: <CURRENT_DOCUMENT> \n\n - Character: <PERSONA>"
\end{minted}


==> prompts_and_confs/str_system_no_copy.tex <==
\begin{minted}[breaklines=true, frame=single, fontsize=\small]{python}
SYSTEM_PROMPT_NO_COPY = "Edit the candidate document to improve its search engine ranking for the candidate query, aiming for the highest rank (1 being the highest). Use the black box search engine's past rankings over various queries, provided as context by the user, to guide your edits. Focus on editing the most impactful sentences to enhance ranking potential. Target an edited document length of around 147 words, not exceeding 150 words. Ensure the edited document is very similar to the candidate document. Generate only the edited document, without additional comments or titles. Don't use a duplicate of another participant's document. Documents that practice this technique will be penalized. However, you are permitted to copy paste parts of documents that other participants have written, As long as the originality of your document is remained.\n Input: \n\n - Candidate Query: <QUERY> \n\n - Candidate Document: <CURRENT_DOCUMENT> \n\n - Character: <PERSONA>"
\end{minted}

==> tables/data_parameters.tex <==
\begin{tabular}{|l|c|}
\hline
\textbf{Parameter} & \textbf{Value(s)} \\
\hline
\textbf{Number of agents} & 4 or 5 \\
\hline
Rounds & 30 \\
\hline
Round by Round & True \\
\hline
Queries & 30 queries selected from TREC \\
\hline
\textbf{Rankers} & intfloat/e5-large-unsupervised, facebook/contriever, Okapi BM25 \\
\hline
\textbf{LLM models of agents} & 
\begin{tabular}[t]{@{}l@{}}
\small{meta-llama/Meta-Llama-3.1-8B-Instruct, google/gemma-2-9b-it,} \\
\small{Qwen/Qwen2.5-7B-Instruct, mlx-community/Ministral-8B-Instruct-2410-bf16}
\end{tabular} \\
\hline
LLM parameters & $top_p = 0.9 ; Temperature = 0.5$ \\
\hline
Characters & BSc student, professional writer, professional editor, \\
& English student, data science professor \\
\hline
Max Tokens & 256 \\
\hline
\textbf{Feedback Mechanism} & Pairwise prompt, listwise prompt\footnote{XX ref to niv} \\
\hline
\textbf{System Prompt} & The system prompt in Bardas et al. \cite{niv} or The the system prompt with addition instruction to not copy. Figures \ref{prompt_system} and \ref{prompt_system_no_copy}\\
\hline
\end{tabular}

==> tables/datasets.tex <==
\begin{tabular}{|l|c|c|c|c|c|}
        \hline
        \textbf{Name} & \textbf{\# Agents} & \textbf{Ranker} & \textbf{LLM Model} & \textbf{Feedback Mechanism} & \textbf{System Prompt} \\ \hline
        Llama E5 Listwise 4 Players & 4 & E5 & Llama3.1 & Listwise & Normal \\ \hline
        Llama E5 Listwise & 5 & E5 & Llama3.1 & Listwise & Normal \\ \hline
        Llama E5 Listwise No Copy & 5 & E5 & Llama3.1 & Listwise & No Copy \\ \hline
        Llama E5 Pairwise 4 Players & 4 & E5 & Llama3.1 & Pairwise & Normal \\ \hline
        Llama E5 Pairwise & 5 & E5 & Llama3.1 & Pairwise & Normal \\ \hline
        Llama E5 Pairwise No Copy & 5 & E5 & Llama3.1 & Pairwise & No Copy \\ \hline
        Gemma E5 Listwise & 5 & E5 & Gemma2 & Listwise & Normal \\ \hline
        Gemma E5 Pairwise & 5 & E5 & Gemma2 & Pairwise & Normal \\ \hline
        Gemma E5 Pairwise No Copy & 5 & E5 & Gemma2 & Pairwise & No Copy \\ \hline
        Ministral E5 Listwise & 5 & E5 & Ministral & Listwise & Normal \\ \hline
        Ministral E5 Pairwise & 5 & E5 & Ministral & Pairwise & Normal \\ \hline
        Qwen E5 Listwise & 5 & E5 & Qwen2.5 & Listwise & Normal \\ \hline
        Qwen E5 Pairwise & 5 & E5 & Qwen2.5 & Pairwise & Normal \\ \hline
        Llama Contriever Listwise & 5 & Contriever & Llama3.1 & Listwise & Normal \\ \hline
        Llama Contriever Listwise No Copy & 5 & Contriever & Llama3.1 & Listwise & No Copy \\ \hline
        Llama3.1 Contriever Pairwise & 5 & Contriever & Llama3.1 & Pairwise & Normal \\ \hline
        Gemma Contriever Listwise & 5 & Contriever & Gemma2 & Listwise & Normal \\ \hline
        Gemma Contriever Pairwise & 5 & Contriever & Gemma2 & Pairwise & Normal \\ \hline
        Llama Okapi Listwise & 5 & Okapi & Llama3.1 & Listwise & Normal \\ \hline
        Llama Okapi Pairwise & 5 & Okapi & Llama3.1 & Pairwise & Normal \\ \hline
        Gemma Okapi Listwise & 5 & Okapi & Gemma2 & Listwise & Normal \\ \hline
        Gemma Okapi Pairwise & 5 & Okapi & Gemma2 & Pairwise & Normal \\ \hline
    \end{tabular}

==> tables/glossary.tex <==
\begin{tabular}{|p{2cm}|p{10cm}|}
\hline
\textbf{Field} & \textbf{Description} \\ 
\hline
game (gid) & A game consists of players competing against each other in a during a fixed number of rounds, and a fixed query and ranker. \\
\hline
competition & A competition comprises a batch of games, each predefined with a different query. \\
\hline
ranker & A function induces a ranking over a set of documents based on a given query that represents the information need. The ranker can be classical (e.g., Okapi) or neural (e.g., E5). \\
\hline
agent & An agent is an entity participating in a competition (i.e multiple games), characterized by properties such as its persona and its method of analyzing feedback from each round of a game. In our simulation, we focus on a specific class of LLM-based agents.  \\
\hline
player & A player is a specific instance of an agent participating in a particular game. \\
\hline
rank & The position of a document within a set of documents submitted by a group of players during a round of a game. \\
\hline
round & Single iteration within a game. In each round, the players analyzes the feedback from previous rounds and modify their candidate documents to aim for the highest ranking. \\
\hline
document id (docno) & An identifier for a document in the competition corpus, uniquely defined by the game (or query), round, and the player who authored the document. \\
\hline
document & A passage of fewer than 256 tokens that a player publishes in a round of a game. \\
\hline
group & A group is the set of players participating in a specific game. \\
\hline
winner & The winner is the player whose document is ranked first in a specific round of a game. \\
\hline
feedback & The rankings of all other players' documents in previous round(s) of the game. \\
\hline
query & Keywords that represent the information need. \\
\hline
query id (qid) & The identifier for a query. \\
\hline
\end{tabular}
